Differential Privacy Has Disparate Impact on Model Accuracy

Differential privacy (DP) is a popular mechanism for training machine learning models with bounded leakage about the presence of specific points in the training data. The cost of differential privacy is a reduction in the model's accuracy. We demonstrate that in the neural networks trained using differentially private stochastic gradient descent (DP-SGD), this cost is not borne equally: accuracy of DP models drops much more for the underrepresented classes and subgroups. For example, a gender classification model trained using DP-SGD exhibits much lower accuracy for black faces than for white faces. Critically, this gap is bigger in the DP model than in the non-DP model, i.e., if the original model is unfair, the unfairness becomes worse once DP is applied. We demonstrate this effect for a variety of tasks and models, including sentiment analysis of text and image classification. We then explain why DP training mechanisms such as gradient clipping and noise addition have disproportionate effect on the underrepresented and more complex subgroups, resulting in a disparate reduction of model accuracy.

==> 7_conclusion.tex <==
\section{Conclusion}

Gradient clipping and random noise addition, the core techniques at the
heart of differentially private deep learning, disproportionately affect
underrepresented and complex classes and subgroups.  As a consequence,
differentially private SGD has disparate impact: the accuracy of a model
trained using DP-SGD tends to decrease more on these classes and subgroups
vs.\ the original, non-private model.  If the original model is ``unfair''
in the sense that its accuracy is not the same across all subgroups,
DP-SGD exacerbates this unfairness.  We demonstrated this effect for
several image-classification and natural-language tasks and hope that
our results motivate further research on combining fairness and privacy
in practical deep learning models.

\paragraphbe{Acknowledgments.}
This research was supported in part by the NSF grants 1611770, 1704296,
1700832, and 1642120, the generosity of Eric and Wendy Schmidt by
recommendation of the Schmidt Futures program, and a Google Faculty
Research Award.

